Primordial non-Gaussianity constraints on dissipative inflation

Dissipative effects appear in many early-Universe scenarios, yet their universal observational signatures and systematic confrontation with data remain largely unexplored. We employ the Open Effective Field Theory of Inflation (Open EFToI) to consistently incorporate dissipative and stochastic effects while preserving scale invariance. Dissipation enhances specific interaction channels of the Goldstone mode, generating distinctive primordial non-Gaussian signatures, beyond those generically produced by standard EFToI. In the weak-dissipation regime, this includes folded bispectrum shapes observationally more favoured than both the equilateral and orthogonal templates. Using the Modal bispectrum pipeline with the Planck CMB data, we obtain the likelihood and derive the first model-independent bounds on early-Universe dissipation. We find a marginalised upper bound on the dissipation scale $\gamma \leq 384\,H$ and a lower bound on the sound speed $c_s \geq 0.38$ at $95\%$ confidence level. The maximum likelihood for best-fit models reveals a degeneracy between $\gamma$ and $c_s$. These results open a model-independent window for probing departures from minimal inflation and discriminating between early-Universe scenarios with stochastic noise and dissipative effects.

==> newcommands.tex <==
%edition
%\newcommand{\ie}{\textsl{i.e.~}}
\newcommand{\ie}{\textsl{i.e.}~}
\newcommand{\cf}{\textsl{cf.}\xspace}
\newcommand{\eg}{\textsl{e.g.}\xspace}
\newcommand{\etal}{\textsl{et al.}\xspace}
%\newcommand{\apriori}{\textsl{a priori~}}
\newcommand{\apriori}{{a priori}\xspace}
\newcommand{\etc}{\textsl{etc.}\xspace}


%math function
\newcommand{\mean}[1]{\left\langle #1 \right\rangle}
\newcommand{\order}[1]{\mathcal{O}\!\left(#1\right)}
\newcommand{\Li}[1]{\mathrm{Li}_{#1}}
\DeclareMathOperator{\Ei}{Ei}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
%\DeclareMathOperator{\erf}{erf}
\newcommand{\Tr}{\mathrm{Tr}}

%larger math symbols
\newcommand{\largemathxl}[1]{{\mathlarger{#1}}}
\newcommand{\largemathxxl}[1]{{\mathlarger{\mathlarger{#1}}}}
\newcommand{\largemathxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{#1}}}}}
\newcommand{\mathlargerxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}
\newcommand{\mathlargerxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}
\newcommand{\mathlargerxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}
\newcommand{\mathlargerxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}}

%alias
\newcommand{\lta}{\lesssim}
\newcommand{\gta}{\gtrsim}
%differential d
\newcommand{\dd}{\mathrm{d}}
%e function
%\newcommand{\ee}{\mathrm{e}}
\newcommand{\ee}{e}


%style
\newcommand{\sss}[1]{{\scriptscriptstyle{#1}}}
\newcommand{\boldmathsymbol}[1]{{\ensuremath{\boldsymbol{#1}}}}

\newcommand{\uPl}{\mathrm{Pl}}
\newcommand{\uin}{\mathrm{in}}
\newcommand{\umin}{\mathrm{min}}
\newcommand{\umax}{\mathrm{max}}
\newcommand{\uend}{\mathrm{end}}
\newcommand{\uini}{\mathrm{ini}}
\newcommand{\ueff}{\mathrm{eff}}
\newcommand{\uinf}{\mathrm{inf}}
\newcommand{\ureh}{\mathrm{reh}}
\newcommand{\urad}{\mathrm{rad}}
\newcommand{\utop}{\mathrm{top}}
\newcommand{\ucri}{\mathrm{cri}}
\newcommand{\ucl}{\mathrm{cl}}
\newcommand{\unuc}{\mathrm{nuc}}
\newcommand{\uobs}{\mathrm{obs}}
\newcommand{\ulim}{\mathrm{lim}}
\newcommand{\uphys}{\mathrm{phys}}
\newcommand{\uPgiP}{\mathrm{(gi)}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\uc}{\mathrm{c}}
\newcommand{\ub}{\mathrm{b}}
\newcommand{\us}{\mathrm{s}}
\newcommand{\uS}{\mathrm{S}}
\newcommand{\uM}{\mathrm{M}}
\newcommand{\uPSP}{(\uS)}
\newcommand{\uV}{\mathrm{V}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uPTP}{(\uT)}
\newcommand{\uE}{\mathrm{E}}
\newcommand{\usssTE}{\sss{\uT \uE}}
\newcommand{\usssS}{\sss{\uS}}
\newcommand{\usssPSP}{\sss{\uPSP}}
\newcommand{\usssT}{\sss{\uT}}
\newcommand{\usssPTP}{\sss{\uPTP}}
\newcommand{\usssPMoneP}{\sss{(\uM=1)}}
\newcommand{\usssPl}{\sss{\uPl}}
\newcommand{\usssRH}{\ureh}
\newcommand{\usssV}{\sss{\uV}}
\newcommand{\usssE}{\sss{\uE}}
\newcommand{\nS}{n_\usssS}
\newcommand{\nT}{n_\usssT}
\newcommand{\alphaS}{\alpha_\usssS}
\newcommand{\alphaT}{\alpha_\usssT}
\newcommand{\one}{{_1}}
\newcommand{\two}{{_2}}
\newcommand{\udm}{\mathrm{dm}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\muS}{\mu_\usssS}
\newcommand{\muT}{\mu_\usssT}
\newcommand{\muST}{\mu_{\usssS,\usssT}}
\newcommand{\uRL}{\mathrm{RL}}
\newcommand{\uNL}{\mathrm{NL}}
\newcommand{\uwkb}{\mathrm{WKB}}

\newcommand{\bmk}{\boldmathsymbol{k}}
\newcommand{\bmp}{\boldmathsymbol{p}}
\newcommand{\bmq}{\boldmathsymbol{q}}
\newcommand{\bmx}{\boldmathsymbol{x}}
\newcommand{\bmy}{\boldmathsymbol{y}}

\newcommand{\ssS}{\mathcal{S}}
\newcommand{\ssE}{\mathcal{E}}
\newcommand{\fnl}{f_{\rm NL}}

\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calI}{\mathcal{I}}

\newcommand{\setR}{\mathbb{R}}
\newcommand{\setC}{\mathbb{C}}

\newcommand{\Rea}{\Re \mathrm{e}\,}
\newcommand{\Ima}{\Im \mathrm{m}\,}

\newcommand{\Real}[1]{\Rea \left[ #1 \right] }
\newcommand{\Imag}[1]{\Ima \left[ #1 \right] }


%units
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\km}{\mathrm{km}}
\renewcommand{\sec}{\mathrm{s}}
\newcommand{\pc}{\mathrm{pc}}
\newcommand{\kpc}{\mathrm{kpc}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\K}{\mathrm{K}}


% General Cosmology

\newcommand{\Hu}{\mathcal{H}}
\newcommand{\Ka}{\mathcal{K}}
\newcommand{\Zed}{\mathcal{Z}}
\newcommand{\cs}{c_{s}}

%cosmo
\newcommand{\omegaT}{\omega_\usssT}
\newcommand{\omegaS}{\omega_\usssS}
\newcommand{\omegaST}{\omega_{\usssS, \usssT}}
\newcommand{\OmegaL}{\Omega_\Lambda}
\newcommand{\OmegaCDM}{\Omega_\udm}
\newcommand{\OmegaB}{\Omega_\ub}
\newcommand{\OmegaR}{\Omega_\gamma}
\newcommand{\Qrms}{Q_{\mathrm{rms-PS}}}
\newcommand{\wstate}{w}
\newcommand{\Mc}{M_\uc}
\newcommand{\potS}{U_{_\uS}}
\newcommand{\potT}{U_{_\uT}}

\newcommand{\mpl}{m_\usssPl}
\newcommand{\Mp}{M_\usssPl}


%inflation
\newcommand{\Hzero}{H_0}
\newcommand{\Hstar}{H_*}
\newcommand{\kstar}{k_*}
\newcommand{\Pstar}{P_*}
\newcommand{\astar}{a_*}
\newcommand{\Pnum}{P^{\usssPMoneP}}
\newcommand{\calNnuc}{\mathcal{N}^\unuc}
\newcommand{\calNend}{\mathcal{N}^\uend}
\newcommand{\calFnuc}{\mathcal{F}^\unuc}
\newcommand{\calFend}{\mathcal{F}^\uend}
\newcommand{\rRL}{r_\uRL}
\newcommand{\csini}{c_{\us \uini}}

\newcommand{\etastar}{\eta_*}
\newcommand{\nustar}{\nu_*}
\newcommand{\csstar}{c_{\us*}}
\newcommand{\epsonestar}{\epsilon_{1*}}
\newcommand{\epstwostar}{\epsilon_{2*}}
\newcommand{\epsthreestar}{\epsilon_{3*}}
\newcommand{\deltaonestar}{\delta_{1*}}
\newcommand{\deltatwostar}{\delta_{2*}}
\newcommand{\epsnstar}{\epsilon_{n*}}
\newcommand{\epsnponestar}{\epsilon_{n+1*}}
\newcommand{\xstar}{x_*}

\newcommand{\ustar}{u_*}
\newcommand{\wstar}{w_*}

\newcommand{\dia}{\sss{\diamond}}
\newcommand{\Hdia}{H_\dia}
\newcommand{\kdia}{k_\dia}
\newcommand{\etadia}{\eta_\dia}
\newcommand{\csdia}{c_{\us \dia}}
\newcommand{\epsonedia}{\epsilon_{1\dia}}
\newcommand{\epstwodia}{\epsilon_{2\dia}}
\newcommand{\epsthreedia}{\epsilon_{3\dia}}
\newcommand{\epsfourdia}{\epsilon_{4\dia}}
\newcommand{\epsfivedia}{\epsilon_{5\dia}}

\newcommand{\deltaonedia}{\delta_{1\dia}}
\newcommand{\deltatwodia}{\delta_{2\dia}}
\newcommand{\deltathreedia}{\delta_{3\dia}}
\newcommand{\deltafourdia}{\delta_{4\dia}}

\newcommand{\grav}{\star}
\newcommand{\Hgrav}{H_\grav}
\newcommand{\kgrav}{k_\grav}
\newcommand{\etagrav}{\eta_\grav}
\newcommand{\epsonegrav}{\epsilon_{1\grav}}
\newcommand{\epstwograv}{\epsilon_{2\grav}}

\newcommand{\aH}{\sss{\circledast}}
\newcommand{\kah}{k_\aH}
\newcommand{\etaah}{\eta_\aH}

\newcommand{\Dwkb}{D_{_\uwkb}}
\newcommand{\Awkb}{A_{_\uwkb}}
%\newcommand{\etaH}{\eta_{_{H}}}


%efolds
\newcommand{\efolds}{$e$-folds~}
\newcommand{\efold}{$e$-fold}
\newcommand{\Nini}{N_\uini}
\newcommand{\Nend}{N_\uend}
\newcommand{\Nreh}{N_\ureh}
\newcommand{\Nstar}{N_*}
\newcommand{\Nzero}{N_\zero}
\newcommand{\Nstarnuc}{N_*^\unuc}
\newcommand{\Nstarend}{N_*^\uend}

\newcommand{\bfk}{\textbf{k}}
\newcommand{\bfq}{\textbf{q}}
\newcommand{\bfp}{\textbf{p}}
\newcommand{\bfx}{\textbf{x}}
%begin and end equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{equation}\begin{aligned}}
\newcommand{\eea}{\end{aligned}\end{equation}}
%\newcommand{\bea}{\begin{align}}
%\newcommand{\eea}{\end{align}}

%figures size
\newlength{\wsingfig}
\setlength{\wsingfig}{0.99\textwidth}
\newlength{\wdblefig}
\setlength{\wdblefig}{0.49\textwidth}
\newlength{\wquadfig}
\setlength{\wquadfig}{0.249\textwidth}
\newlength{\wtriplefig}
\setlength{\wtriplefig}{0.333\textwidth}


% References
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[1]{Eqs.~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~{\ref{#1}}}
\newcommand{\Figs}[1]{Figs.~{\ref{#1}}}
\newcommand{\Refa}[1]{Ref.~{\cite{#1}}}
\newcommand{\Refs}[1]{Refs.~{\cite{#1}}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Secs}[1]{Secs.~\ref{#1}}
\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\Apps}[1]{Appendices~\ref{#1}}

\newcommand{\bs}[1]{\boldsymbol{#1}}




